Anytime Bi-Objective Optimization with a Hybrid Multi-Objective CMA-ES (HMO-CMA-ES)

We propose a multi-objective optimization algorithm aimed at achieving good anytime performance over a wide range of problems. Performance is assessed in terms of the hypervolume metric. The algorithm called HMO-CMA-ES represents a hybrid of several old and new variants of CMA-ES, complemented by BOBYQA as a warm start. We benchmark HMO-CMA-ES on the recently introduced bi-objective problem suite of the COCO framework (COmparing Continuous Optimizers), consisting of 55 scalable continuous optimization problems, which is used by the Black-Box Optimization Benchmarking (BBOB) Workshop 2016.

==> pprldmany-single-functions/pprldmany.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_1-separable_1-separable.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_1-separable_2-moderate.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_1-separable_3-ill-conditioned.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_1-separable_4-multi-modal.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_1-separable_5-weakly-structured.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_2-moderate_2-moderate.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_2-moderate_3-ill-conditioned.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_2-moderate_4-multi-modal.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_2-moderate_5-weakly-structured.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_3-ill-conditioned_3-ill-conditioned.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_3-ill-conditioned_4-multi-modal.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_3-ill-conditioned_5-weakly-structured.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_4-multi-modal_4-multi-modal.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_4-multi-modal_5-weakly-structured.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_5-weakly-structured_5-weakly-structured.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f001.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f002.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_f003.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f004.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f005.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_f006.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f007.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f008.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f009.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f010.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f011.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f012.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f013.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f014.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_f015.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f016.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f017.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f018.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_f019.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_f020.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f021.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}}}


==> pprldmany-single-functions/pprldmany_f022.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f023.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_f024.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_f025.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f026.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f027.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f028.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f029.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f030.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f031.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_f032.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f033.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f034.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f035.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f036.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f037.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f038.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f039.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_f040.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f041.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f042.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_f043.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_f044.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f045.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_f046.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_f047.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}}}


==> pprldmany-single-functions/pprldmany_f048.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f049.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f050.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_f051.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f052.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}}}


==> pprldmany-single-functions/pprldmany_f053.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}}}


==> pprldmany-single-functions/pprldmany_f054.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}}}


==> pprldmany-single-functions/pprldmany_f055.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{2-D}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{3-D}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{5-D}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{10-D}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{20-D}{\nperfprof}}\providecommand{\perfprofsidepanel}{{\mbox{\algEperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}}}

